Finding Your Voice: The Linguistic Development of Mental Health Counselors

Mental health counseling is an enterprise with profound societal importance where conversations play a primary role. In order to acquire the conversational skills needed to face a challenging range of situations, mental health counselors must rely on training and on continued experience with actual clients. However, in the absence of large scale longitudinal studies, the nature and significance of this developmental process remain unclear. For example, prior literature suggests that experience might not translate into consequential changes in counselor behavior. This has led some to even argue that counseling is a profession without expertise. In this work, we develop a computational framework to quantify the extent to which individuals change their linguistic behavior with experience and to study the nature of this evolution. We use our framework to conduct a large longitudinal study of mental health counseling conversations, tracking over 3,400 counselors across their tenure. We reveal that overall, counselors do indeed change their conversational behavior to become more diverse across interactions, developing an individual voice that distinguishes them from other counselors. Furthermore, a finer-grained investigation shows that the rate and nature of this diversification vary across functionally different conversational components.

==> FIG/030_cc_hist.tex <==
% !TEX root = ../paper-main.tex
\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{FIG/DRAFT/030_cc_hist.png}
\caption{\todo{Histogram of counselor tenures.}}
\label{fig:cc_hist}
\end{figure}


==> FIG/050_increase_heatmap.tex <==
% !TEX root = ../paper-main.tex
\begin{figure*}[t]
\centering
\includegraphics[width=0.8\textwidth]{FIG/increase_heatmap.png}
\caption{
Temporal diversification trends across different counselor life-stages (left to right). Each cell shows the percentage of counselors that increase in diversity from that 
% respective 
life-stage to their tenured life-stage \maxlifestage; *'s indicate statistical significance (binomial test $p<0.05$, comparing to 50\% by chance).  The topmost row shows the temporal trend across the entire conversation, and the subsequent rows separate this trend by conversational component.  
}
\label{fig:increase_heatmap}
\end{figure*}


==> FIG/050_seg_word_egs.tex <==
% !TEX root = ../paper-main.tex


\begin{table*}[]
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Component}  & \textbf{Description}                                                                                        & \textbf{Example words}                                                           \\ \midrule
\small \firstseg               &\small greeting the texter and building rapport                                                                    &\small \begin{tabular}[c]{@{}l@{}}\egword{hi}, \egword{name}, \egword{listen}, \egword{contacting}\end{tabular}                                                                \\ \midrule
\small \secondseg &\small \begin{tabular}[c]{@{}l@{}}understanding texter concerns  and precipitating events\end{tabular}     &\small \begin{tabular}[c]{@{}l@{}}\egword{past}, \egword{anyone},  \egword{relationship}, \egword{diagnosed}   \end{tabular}                                                \\ \midrule
\small\thirdseg &\small \begin{tabular}[c]{@{}l@{}}understanding texter motivations  and past attempts to cope\end{tabular} &\small \begin{tabular}[c]{@{}l@{}}\egword{tried}, \egword{brainstorm},  \egword{needs}, \egword{psychiatrist}\end{tabular} \\ \midrule
\small\fourthseg     &\small \begin{tabular}[c]{@{}l@{}}collaborating with the texter  to come up with next steps\end{tabular}         &\small \begin{tabular}[c]{@{}l@{}}\egword{music}, \egword{favorite}, \egword{meditation}, \egword{apps}                                        \end{tabular}               \\ \midrule\small
\fifthseg             &\small summarizing and closing the conversation            & \small\begin{tabular}[c]{@{}l@{}}\egword{care}, \egword{night}, \egword{welcome}, \egword{anytime}\end{tabular}                                                           \\ \bottomrule
\end{tabular}
\caption{
Functional components of counseling conversations, as delineated by successive fifths of a conversation. Descriptions of these components are adapted from the counselor training textbook; 
example words are taken from those which are particularly frequent in the corresponding fifth of the conversation compared to overall, as described in Section \ref{sec:lexical}.
}
\label{tab:seg_word_egs}
\end{table*}

==> FIG/051_entry_idx_hist.tex <==
% !TEX root = ../paper-main.tex
\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{FIG/DRAFT/051_entry_idx_hist.png}
\caption{
	The distribution of median entry indexes of words used by tenured counselors. Bolded line denotes the median entry index (64); dotted lines mark lower and upper quartiles.
}
\label{fig:entry_idx_hist}
\end{figure}


==> FIG/051_word_egs.tex <==
% !TEX root = ../paper-main.tex
\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{FIG/DRAFT/051_word_egs.png}
\caption{
	The distribution of median entry indexes of tenured counselors' words, separated by conversational components; along with example words from each segment at various entry indexes. (Compare with baseline distribution in Figure \ref{fig:entry_idx_hist}.)
	Words are ordered by, and colored according to their median entry index, such that green words tend to be first used earlier in a counselor's tenure while brown words tend to be first used later on.
}
\label{fig:word_egs}
\end{figure*}


==> FIG/usage_shift.tex <==
% !TEX root = ../paper-main.tex
\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{FIG/usage_shift.png}
\caption{
	\camerareadynew{The distribution of usage shifts of the 
	%%C0609: not sure we need to repeat this
	%	3461 words used by at least 20\% of counselors. 
	words making up the core counselor vocabulary (i.e., used by at least 20\% of counselors).
	 Dashed line denotes the median usage shift.}
	% The distribution of usage shifts of words used by counselors. Dashed line denotes the median usage shift 
	%%C0606: edit
	%	(0.011).
	%%J0607: I slightly tweaked the selection criterion -- now it's ``used by at least 20% of ccs again. maybe it's not even worth listing?'
	% (0.002).
}
\label{fig:usage_shift_hist}
\end{figure}


==> FIG/usage_shift_segs.tex <==
% !TEX root = ../paper-main.tex
\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{FIG/usage_shift_combined.pdf}
\caption{
	\textbf{Top}: the overall distribution of usage shifts of the words 
	% making up the core 
	\camerareadynew{at the core of the}
	counselor vocabulary (i.e., used by at least 20\% of counselors). 
	\textbf{Bottom}: 
	% considering only the 
	\camerareadynew{usage shift distributions per}
	subset of words characteristic to each conversational component, along with examples.
	Words are ordered by, and colored according to their usage shift, such that blue words tend to be used more by counselors in their earlier conversations while red words tend to be used more by counselors with more experience.
	%%C0606: added
	Dashed lines indicate the respective medians.
}
\label{fig:usage_shift_hist_segs}
\end{figure*}

%%C0609: before joinig figures
%
% The distribution of usage shifts 
% 	%%C0606: edit
% 	%	of counselors' words, separated by conversational components;
% 	for counselor words characteristic to each conversational component, 
% 	 along with examples.
% 	 %%C0606: i think it's repetitive
% 	  %	  ; along with example words from each segment with various shifts.
% 	  (Compare with baseline distribution in Figure \ref{fig:usage_shift_hist}.)
% 	Words are ordered by, and colored according to their usage shift, such that blue words tend to be used more by counselors in their earlier conversations while red words tend to be used more by counselors with more experience.
% 	%%C0606: added
% 	Dashed lines indicate the respective medians.
